Implicit Regularization of Discrete Gradient Dynamics in Linear Neural Networks

When optimizing over-parameterized models, such as deep neural networks, a large set of parameters can achieve zero training error. In such cases, the choice of the optimization algorithm and its respective hyper-parameters introduces biases that will lead to convergence to specific minimizers of the objective. Consequently, this choice can be considered as an implicit regularization for the training of over-parametrized models. In this work, we push this idea further by studying the discrete gradient dynamics of the training of a two-layer linear network with the least-squares loss. Using a time rescaling, we show that, with a vanishing initialization and a small enough step size, this dynamics sequentially learns the solutions of a reduced-rank regression with a gradually increasing rank.

==> defs.tex <==
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\Sp}{Sp} % Spectrum
\DeclareMathOperator*{\sri}{sri}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\loss}{loss}
\DeclareMathOperator*{\relint}{relint}
\DeclareMathOperator*{\Fix}{{Fix}}
\DeclareMathOperator*{\domain}{dom}
\DeclareMathOperator{\prox}{\mathbf{prox}}
\DeclareMathOperator{\thinprox}{prox}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\Err}{Err}
\newcommand{\bigzero}{\mbox{\normalfont\Large\bfseries 0}}


\definecolor{mygreen}{rgb}{0.032, 0.6392, 0.2039}
\newcommand{\cmark}{\textcolor{mygreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}

\usepackage{todonotes}
\newcommand{\mytodo}[2][]{\todo[inline,color=babyblueeyes,#1]{#2}}

\def\RR{{\mathbb R}}
\def\NN{{\mathbb N}}
\def\EE{{\mathbb E}}
\def\DD{{\boldsymbol{\Delta}}}

% \def\prox{{\mathbf{prox}}}
% \def\eprox{{\emph{\text{prox}}}}
\def\xx{{\boldsymbol x}}
\def\XX{{\boldsymbol X}}
\def\ZZ{{\boldsymbol Z}}
\def\YY{{\boldsymbol Y}}
\def\uu{{\boldsymbol u}}
\def\UU{{\boldsymbol U}}
\def\rr{{\boldsymbol r}}
\def\ww{{\boldsymbol w}}
\def\yy{{\boldsymbol y}}
\def\vv{{\boldsymbol v}}
\def\ww{{\boldsymbol w}}
\def\zz{{\boldsymbol z}}
\def\KK{{\boldsymbol K}}
\def\CC{{\boldsymbol C}}
\def\TT{{\boldsymbol T}}
\def\LL{{\mathcal L}}
\def\X{{\mathcal X}}
\def\balpha{{\boldsymbol u}}
\def\defas{:=}

\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{axiom}{Axiom}


\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{
\newenvironment{rep#1}[1]{
 \def\rep@title{#2 \ref{##1}}
 \begin{rep@theorem}}
 {\end{rep@theorem}}}
\newreptheorem{theorem}{Theorem'}
\binoppenalty=10000
\relpenalty=10000

\newtheorem*{rep@proposition}{\rep@title}
\newcommand{\newrepproposition}[2]{
\newenvironment{rep#1}[1]{
 \def\rep@title{#2 \ref{##1}}
 \begin{rep@proposition}}
 {\end{rep@proposition}}}
\newreptheorem{proposition}{Proposition'}
\binoppenalty=10000
\relpenalty=10000
